Survey of Transient Execution Attacks

Transient execution attacks, also called speculative execution attacks, have drawn much interest as they exploit the transient execution of instructions, e.g., during branch prediction, to leak data. Transient execution is fundamental to modern computer architectures, yet poses a security risk as has been demonstrated. Since the first disclosure of Spectre and Meltdown attacks in January 2018, a number of new attack types or variants of the attacks have been presented. These attacks have motivated computer architects to rethink the design of processors and propose hardware defenses. This paper summarizes the components and the phases of the transient execution attacks. Each of the components is further discussed and categorized. A set of metrics is proposed for each component to evaluate the feasibility of an attack. Moreover, the data that can be leaked in the attacks are summarized. Further, the existing attacks are compared, and the limitations of these attacks are discussed based on the proposed metrics. In the end, existing mitigations at the micro-architecture level from literature are discussed.

==> Makefile <==
RM     := /bin/rm -rf

all:
	@echo "\nUse 'make conf' to build arXiv paper.\n"

paper: 
	pdflatex main ; bibtex main; pdflatex main; pdflatex main;

conf:
	pdflatex main-sigconf ; bibtex main-sigconf; pdflatex main-sigconf; pdflatex main-sigconf;

quick:
	pdflatex main-sigconf

clean: 
	$(RM) *.dvi paper.ps *.log *.aux main.pdf *.blg *.bbl *~* main.out main-sigconf.pdf  main-sigconf.out *.gz

rmtrailingspaces:

	sed -i.bak '/^[[:blank:]]*%/d' main-sigconf.tex
	sed -i.bak '/^[[:blank:]]*%/d' abstract.tex
	sed -i.bak '/^[[:blank:]]*%/d' intro.tex
	sed -i.bak '/^[[:blank:]]*%/d' background.tex
	sed -i.bak '/^[[:blank:]]*%/d' threat_model.tex
	sed -i.bak '/^[[:blank:]]*%/d' components.tex
	sed -i.bak '/^[[:blank:]]*%/d' transient_exe.tex
	sed -i.bak '/^[[:blank:]]*%/d' covert_channel.tex
	sed -i.bak '/^[[:blank:]]*%/d' transient_attacks.tex
	sed -i.bak '/^[[:blank:]]*%/d' mitigations.tex
	sed -i.bak '/^[[:blank:]]*%/d' related_attacks.tex
	sed -i.bak '/^[[:blank:]]*%/d' conclusion.tex

	sed -i.bak 's/[[:blank:]]*$$//' main-sigconf.tex
	sed -i.bak 's/[[:blank:]]*$$//' abstract.tex
	sed -i.bak 's/[[:blank:]]*$$//' intro.tex
	sed -i.bak 's/[[:blank:]]*$$//' background.tex
	sed -i.bak 's/[[:blank:]]*$$//' threat_model.tex
	sed -i.bak 's/[[:blank:]]*$$//' components.tex
	sed -i.bak 's/[[:blank:]]*$$//' transient_exe.tex
	sed -i.bak 's/[[:blank:]]*$$//' covert_channel.tex
	sed -i.bak 's/[[:blank:]]*$$//' transient_attacks.tex
	sed -i.bak 's/[[:blank:]]*$$//' mitigations.tex
	sed -i.bak 's/[[:blank:]]*$$//' related_attacks.tex
	sed -i.bak 's/[[:blank:]]*$$//' conclusion.tex
	rm *.bak


==> background.tex <==
\section{Background}
\label{sec:background}

This section gives background about various optimizations in micro-architecture
that lead to the transient execution, and thus in turn contribute to the transient execution attacks.
Many more details about CPU micro-architecture and pipeline details available in architecture textbooks, e.g.,~\cite{hennessy2011computer}.
This section also discusses conventional side channels and covert channels based on timing;
many more details about the timing channels are given in other surveys, e.g.,~\cite{szefer2018survey}.
The two concepts combined lead to the transient execution attacks, which
is the topic of the rest of this survey.

\subsection{Performance Optimizations that Enable Transient Execution Attacks}
\label{sec:background_perf_opt}

Due to the data dependencies between instructions, the CPU pipeline sometimes has to stall until the dependencies are resolved.
To reduce the stalls in the pipeline and to keep the pipeline full, many performance-improving and area-reducing optimizations have been proposed and implemented
in today's commodity processors.

\textbf{Out-of-Order Execution (OoO):}
In OoO, some of the younger instructions can be executed earlier than the older instructions (based on program order) if all the dependencies of the younger instructions are available.
OoO helps to improve instruction-level parallelism.
\hl{In OoO, the life cycle of instruction is: fetch, dispatch, issue (a.k.a. execute), and retire (a.k.a. commit).
The instruction is first fetched to the pipeline, and after decoding, micro-ops are dispatched.
Once all the dependencies of the instruction are satisfied, an instruction (or micro-op) is issued for execution. 
OoO uses a reorder buffer (ROB) to hold the instructions (or micro-ops) and execution results and to retire each instruction (or micro-op)
in the program order.  Instructions (or micro-ops) are retired (committed) when they reach the head of ROB.}
%\textbf{TODO: are there any ROB-based channels?}
%Because of OoO execution, some instructions can take more time to execute while they wait for data or functional units to be available, leading to timing differences.

\textbf{Speculative Execution:}
Speculative execution occurs when there is a control flow instruction for which the processor does not know the result yet.
For example, a branch condition needs to be computed before the branch result (taken or not taken) can be obtained.
To improve performance, processors often speculate the outcome of such instructions and begin to execute instructions down
the speculated path.  Later, either speculation is confirmed to be correct, or there is a mis-speculation, and instructions that began to execute down the mis-speculated path are squashed (cleared from the pipeline).  
After mis-speculation, the processor should clean up all architectural and micro-architectural state
to create an illusion as if these instructions never executed.
In addition to control flow, speculation is used whenever there are other types of prediction, such as prefetching
or value prediction (not used in commodity processors).
%Because of the speculation, instructions may take different amount of time based on correct or incorrect speculation results.

\textbf{Delayed Fault Validation:}
Similar to speculation for control flow, processors speculate that there is no fault and continue execution even when there is a potential fault.
Especially, fault checking can be delayed, and some processors allow for instructions to continue executing
during which time the data (that should have been inaccessible due to the fault) can be accessed and micro-architecture states can be modified.  If there is any fault, the processor then should clean up all the architectural and micro-architectural state changes.

\textbf{Caching:}
One of the key optimizations for memory-related operations is caching.  Modern processors
have multiple levels of caches, typically L1, L2, and Last Level Cache (LLC). 
%The caches can be inclusive, non-inclusive, or exclusive.
%Most processors have inclusive or non-inclusive caches (data in a higher-level cache may or may not be in a lower level; in contrast, in exclusive
%caches, data in higher level cache is never in lower level).
A cache hit occurs when data is found in a cache, and the processor does not need to go to the main memory to fetch the data.
Based on the level of cache where data is found, it can be up to about $500\times$ faster to get data if it is a hit.
Other cache-like structures exist in processors, such as TLBs, which can also offer performance improvement by caching data.

\textbf{Sharing of Functional Units in Hyper-Threading within a Processor Core:}
To reduce the area and power consumption, functional units are shared among hardware threads in hyper-threading.
Today, most processors are built with two-thread SMT (Simultaneous Multi-Threading) configurations.
In SMT, in the execution stage, the processor decides with instructions from which threads can execute
based on the available execution units.  It is expected that not all programs need all the units at the same time, so the sharing allows for good performance
while reducing the need to duplicate all units among all SMT threads.

\textbf{Sharing of Resources Among Cores in Multi-Core Processors:}
Similar to sharing within the processor core, many resources are shared among cores.
These include caches,  prefetchers, various buffers, memory controllers, directories, and other cache coherence related structures,
memory busses, I/O, etc.  Rather than each core having a separate one of these units, they are shared to reduce hardware resources.

\subsection{Covert and Side Channels}

\begin{figure}[t]
\includegraphics[width=3.2in]{gfx/side_and_covert_channel_background-crop.pdf}
\caption{\small Components of a side or covert channel: (a) a sender in a covert channel, also called victim in a side channel;
(b) and (c) a change in state of the processor; and (d) receiver in the side or a covert channel.}
 \label{fig:side_and_covert_channels_bkg}
\end{figure}

Figure~\ref{fig:side_and_covert_channels_bkg} shows the components of a typical side or covert channel.
First, there is the entity sending (or leaking) the information.  Commonly this entity is called the sender in covert channels, and the victim
in side channels.  Execution of some instructions by the sender causes the state of the processor to be modified.
The states can be internal processor states or physical states such as temperature or EM emanations.
Finally, the receiver observes the state change to learn about a bit of information transmitted by the sender.

In timing channels, which are the focus of this survey, the focus is on changes in the processor, which can be observed by
software through measurements of the execution time of some operations, Figure~\ref{fig:side_and_covert_channels_bkg} (c).
The state modification can be the architectural state or the micro-architectural state.  However, because by design processors
do not leak any information from the architectural state (e.g., two processes in different memory spaces cannot access each other's memory),
majority of the timing channels abuse the micro-architectural state changes, which cannot be directly read,
but which can be observed through timing differences. These covert channels are the result of the various performance optimizations
discussed in Section~\ref{sec:background_perf_opt}. There are currently only limited hardware features that are designed to defend against covert channels, e.g., Intel Cache Allocation Technology (CAT)~\cite{liu2016catalyst}, and many covert channels remain open.
%Note that senders instructions can be executed ``on-purpose'' as part of the application's normal operation,
%or they can be executed during speculation, as transient instructions which may or may not be eventual squashed depending on
%the outcome of
%the speculation or prediction.
%For the channels, some instruction needs to execute to modify the processor state, and how it is executed is a separate issue.

%This creates a possible distinction between {\em conventional channels} based on timing where the instructions are executed on-purpose,
%and {\em transient execution channels} based on timing where the instructions of the sender are executed during transient execution;
%but nevertheless modify the state of the processor and that state is not cleaned up.





==> future_work.tex <==
\section{Open Research Challenges}
\label{sec:future_work}

One research direction is to further discover new attacks. Since the detailed designs of commercial processors are not public, there might be unknown attacks. 
There could be more data that is exploitable in transient execution. In Spectre-type attacks, as shown in Table~\ref{tbl:privilege_level}, we assume the victim is executing transiently and the attacker then can access data that the victim could access architecturally. 
As demonstrated in Spectre V1 attack using SWAPGS instruction~\cite{swapgs}, the attacker can learn data that the victim could access architecturally even after context switch. 
The security boundaries that are broken in the attacks depend on the implementation, and can be explored in the future.
Meanwhile, there could also be new covert channels in the micro-architecture.
As shown in Table~\ref{tbl:attack_demo}, new combinations of transient execution and covert channel can be demonstrated for different attack scenarios.

Another research direction is to design hardware to defend the transient execution attacks. 
Transient execution is critical to the performance of processors and is also the root cause of the attacks.
A couple of mitigation strategies are proposed and discussed in Section~\ref{sec:mitigations}.  
Proposals and optimization to defend the attack with lower performance overhead are desired. 
The mitigations can come with different threat models to provide a trade-off between performance and security. 

The transient execution attacks also affect the formal analysis of software behavior. In the past, the software analysis is either based on software semantics or an ISA level hardware model. To analyze the transient execution attacks rigorously, a formal micro-architecture level or RTL level model is required. ~\cite{cryptoeprint:2019:310,mcilroy2019spectre,guarnieri2018spectector} shed light on this direction.

==> related_attacks.tex <==
\section{Other Attacks Leveraging Transient Execution}
\label{sec:related_attacks}

Another category of attacks that can be mistaken with the transient execution attacks is the covert channel attacks leveraging transient execution.
Different from the transient execution attacks where the goal of the attacker is to compromise the confidentially of victim's secret,  these attacks have the goal to build  novel covert channels leveraging the hardware units for transient execution~\cite{evtyushkin2018branchscope,evtyushkin2015covert,evtyushkin2016jump,Islam2018SPOILER}, such as the branch prediction unit, STL, etc.

Modern computer architectures gain performance benefits from transient execution.
Correct predictions result in useful transient execution results and make the execution faster. When a wrong prediction is made, the results of transient execution will be discarded and sometimes cause a small penalty.
Therefore, there is a time difference in the execution due to transient execution, and a timing-based covert channel can be built.

As shown in Table~\ref{tbl:pred_share}, prediction units are shared between different users. The sender can train a prediction unit, and then the receiver can observe different prediction results.
Real covert channel attacks have been demonstrated by leveraging the prediction units, such as {\em Branchscope} attack, which uses PHT~\cite{evtyushkin2018branchscope,evtyushkin2015covert,yu2019speculative},  {\em Jump over ASLR}, which uses BTB~\cite{evtyushkin2016jump,weisse2019nda}, and {\em Spoiler} attack which uses STL~\cite{Islam2018SPOILER}.
Other than building covert channel across processes and SGX enclave~\cite{evtyushkin2018branchscope},
these attacks also break KASLR (Kernel address space layout randomization)~\cite{evtyushkin2016jump} and
leak the physical address mapping~\cite{Islam2018SPOILER}.


==> threat_model.tex <==


\section{Threat Model}
\label{sec:threat_model}


The existing transient execution attacks have various threat models. 
In this section, we summarize the attacker's goals and assumptions on the attacker (e.g., the levels of hardware sharing between the attacker and the victim) in the existing attacks. 
Later, we use the assumptions defined in this section when we discuss the attack components.

\subsection{Attacker's Goal: Breaking Security Boundaries}
\label{sec:attacker_goal}

\begin{figure}[t]
\includegraphics[width=4in]{gfx/security_boundary-crop.pdf}
\caption{\small Security boundaries in computer systems that are broken by transient execution attacks.}
\label{fig:security_boundary}
\end{figure}


There are many security boundaries (between different privilege levels or security domains) in a typical processor, as shown in Figure~\ref{fig:security_boundary}.
The goal of the attacker of the transient execution attacks is to cross the security boundaries to obtain information related to the victim's secret data. 
%The victim's secret data here refers to any data that is not accessible to the attacker directly.
%e.g., kernel memory page that should be not accessible to a user-level attacker or SGX enclave data that should not be gotten from outside of the enclave.
We categorize the possible privilege levels or security domains where the attack can originate, shown as red arrows in Figure~\ref{fig:security_boundary}, and wherefrom it is trying to extract data as follows:
\begin{enumerate} %[itemindent=15pt,leftmargin=0pt,listparindent=\parindent]
\item \textbf{user-level program attacking another user-level program:}
The attacker and the victim are two separate user applications, \hl{e.g., the attacker process tries to learn the memory content of another process}. \cite{bhattacharyya2019smotherspectre} \hl{demonstrates when an victim OpenSSH server process is running, how an attacker process learns the host private key.}

\item \textbf{user-level program attacking the kernel:}
The attacker runs in the user level and wants to read the privileged data of the kernel, \hl{e.g., }\cite{Lipp2018meltdown}\hl{ demonstrate an attack that dumps kernel memory from an unprivileged application.}

\item \textbf{virtual machine attacking another virtual machine:}
The attacker and the victim reside in two different guest virtual machines, \hl{e.g.,} \cite{bhattacharyya2019smotherspectre}\hl{ shows it is possible for an attacker VM to learn the private key of OpenSSH server in victim VM.} 
\item \textbf{virtual machine attacking the hypervisor:}
\hl{The attacker is a guest OS and the victim is the host hypervisor e.g.,}~\cite{Kocher2018spectre}\hl{ demonstrate an attack against KVM that leaks host memory when the attacker has full control of the OS inside VM.}

\item \textbf{code running outside an enclave attacking victim running inside an enclave:}
The victim runs inside a security domain protected by some hardware scheme, e.g., SGX enclaves~\cite{costan2016intel}, XOM~\cite{lie2000architectural}, Aegis~\cite{suh2014aegis}, Bastion~\cite{champagne2010scalable}, Sanctum~\cite{costan2016sanctum} or Keystone~\cite{lee2019keystone}, and the attacker code runs outside of it. 
%Since SGX is the only commercial architecture, we use the enclave as an example. 
~\cite{chen2018sgxpectre} \hl{demonstrated such an attack that retrieves secret inside the SGX enclave.}


\item \textbf{attacks across security domains protected by software:}
The victim runs inside the security domain protected by some software scheme, e.g., sandboxes in JavaScript, and the attacker code runs outside of it, as shown in~\cite{Kocher2018spectre}.

\end{enumerate}

In addition, some attacks focus on \textbf{Stale Data} stored somewhere in hardware, e.g., data remaining in registers buffers after it should have been cleaned up~\cite{v4}.
%Sometimes the stale data points to a secret address that the attack want to access.
Sometimes the stale data is of a different privilege level or security domain, so the attacker will break the security domain when accessing stale data.

\hl{Existing transient execution attacks can break all of the security boundaries above. Details will be discussed in Section}~\ref{sec:consequence}, especially in Table~\ref{tbl:privilege_level}.

\subsection{Level of Hardware Sharing}
\label{sec:colocation_attacker}

\hl{The transient execution attacks relies on attacker's ability to access the micro-architectural states that contains victim's information.}
%If there is only the attacker running, the location of the attacker does not matter.
If there are both the attacker and the victim running, \hl{it is assumed the attacker can co-locate with the victim. The attack can be launched in a variety of settings.}
The attacker and the victim could share the hardware in the following settings:
\begin{itemize}
\item \textbf{Same thread:}  running on  the same logical core (hardware thread) in a time-sliced setting, and there might be  context switches in between.
\item \textbf{Same core, simultaneous multithreading (SMT):}  running on different logical cores (hardware threads) on the same physical core.
\item \textbf{Same chip, different core:} sharing LLC, memory bus, and other peripheral devices.
\item \textbf{Same motherboard:} sharing memory bus and peripheral devices.

\end{itemize}

%(T) same logical core (hardware thread)--on same thread on same core  (but not necessarily time-slice.)
%
%(S) same physical core (SMT case)-- on seprate hardware threads in same core
%
%(C) same chip, different cores -- as name implies
%
%(M) same motherboard, different processors -- as name implies

\hl{In some Spectre-type attacks, the speculation of the victim can be controlled by the attacker when the attacker is able to train the prediction unit. In this case, the attack must be able to share the prediction unit (entry) with the victim. We will discuss the level of sharing needed to use different prediction unit in Table}~\ref{tbl:pred_share} in Section~\ref{sec:transient_exe}.
\hl{Covert channels also relies on sharing of hardware components. When the attacker and the victim share different components, different covert channels can be used. More details will be discussed in Table}~\ref{tbl:channel_share} in Section~\ref{sec:covert_channel}. 
\hl{Colocating is not a trivial task. An attack is more feasible when less sharing is required.}



\subsection{Address Space of the Attacker}
\label{sec:addr_space_attacker}
%The attacker and the victim needs to share hardware components for covert channel and the prediction unit for the Spectre-type attacks.
%Some hardware components have many entries and the attacker and the victim need to share the same entry,  e.g., in caches, branch prediction unit (BPU). These entries are indexed by either physical address, virtual address, or a function of the address.
%If the entry is indexed by the physical address or a function of the physical address, the attacker needs to share some physical address with the victim. 
%In that case, if the attacker and the victim are in different address spaces without any shared memory the attack will not be possible.
The attacker's and the victim's address space can be one of the following:
\begin{itemize}
\item \textbf{In the same address space:} In this case, the attacker and the victim have the same virtual to physical address mapping.
\item \textbf{In different address spaces with shared memory:} In this case, the attacker and the victim have different virtual to physical address mappings. But some of the attacker's pages and the victim's pages map to the same physical pages. This can be achieved by sharing dynamic libraries (e.g., libc).
\item \textbf{In different address spaces without shared memory:} The attacker and the victim have different virtual to physical address mapping. And their physical addresses do not overlap.
\end{itemize}


\hl{During the attack, the attacker and the victim need to share the same entry of hardware component to mis-train the prediction unit or for covert channel. To share the same entry, the attacker need to control the address to map to the same entry as the victim. The required address space for the attacker in mis-training will be listed in Table}~\ref{tbl:pred_share} in Section~\ref{sec:transient_exe}.


